Observation of direct CP violation in the measurement of the Cabibbo-Kobayashi-Maskawa angle gamma with B+- --> D(*)K(*)+- decays

We report the determination of the Cabibbo-Kobayashi-Maskawa CP-violating angle gamma through the combination of various measurements involving B^{+-} --> D K^{+-}, B^{+-} --> D^{*} K^{+-}, and B^{+-} --> D K^{*+-} decays performed by the BaBar experiment at the PEP-II e^{+}e^{-} collider at SLAC National Accelerator Laboratory. Using up to 474 million B\bar{B} pairs, we obtain gamma = (69 ^{+17}_{-16})^\circ (modulo 180^\circ). The total uncertainty is dominated by the statistical component, with the experimental and amplitude-model systematic uncertainties amounting to +-4^\circ. The corresponding two-standard-deviation region is 41^\circ < gamma < 102^\circ. This result is inconsistent with gamma = 0 with a significance of 5.9 standard deviations.

==> babarsym.tex <==
%%%%   Standard symbols for use in BABAR papers and BAD Notes
%%%%%
%%%%%   Revised    12/7/00 D. Hitlin      Added features of D. Kirkby's HEP.sty
%%%%%   Revised    7/13/00 R. Waldi       Corrected \Kbar, \Bbar ... macros
%%%%%   Revised    7/13/00 D. MacFarlane  Replaced incorrect \chic1 symbols
%%%%%   Revised    7/05/00 P. Dauncey     Added \mes, \mec, removed \O
%%%%%   Revised    7/04/00 D. MacFarlane  Added scalable version of BABAR
%%%%%   Revised    7/01/00 D. MacFarlane
%%%%%   Revised    6/21/00 D. Hitlin
%%%%%   Original   6/10/00 D. Hitlin
%%%%%   Revision of TDR and Physics Book symbol file
%%%%%

\RequirePackage{xspace}

%%%%%%%%%%%%%%%%%%%% BABAR ... THE NAME OF THE COLLABORATION %%%%

% Huge boldface
\def\hbabar{\mbox{{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A}\hspace{-0.03em}{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A\hspace{-0.03em}R}}}
% LARGE
\def\Lbabar{\mbox{{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A}\hspace{-0.07em}{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A\hspace{-0.02em}R}}}
% Large
\def\lbabar{\mbox{{\large\sl B}\hspace{-0.4em} {\normalsize\sl A}\hspace{-0.03em}{\large\sl B}\hspace{-0.4em} {\normalsize\sl A\hspace{-0.02em}R}}}
% normal size
%\def\babar{\mbox{\sl B\hspace{-0.4em} {\small\sl A}\hspace{-0.37em} \sl B\hspace{-0.4em} {\small\sl A\hspace{-0.02em}R}}}
% replace normalsize with scalable version       dbm 7/4/00
\usepackage{relsize}
\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
    B\kern-0.1em{\smaller A\kern-0.2em R}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{e}\xspace}
\def\en         {\ensuremath{e^-}\xspace}      % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}\xspace}
\def\epm        {\ensuremath{e^\pm}\xspace} 
\def\epem       {\ensuremath{e^+e^-}\xspace}
\def\ee         {\ensuremath{e^-e^-}\xspace}
\def\mmu        {\ensuremath{\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace}    % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace}
\def\mtau       {\ensuremath{\tau}\xspace}
\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}
\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace}
\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
\def\nuenueb    {\ensuremath{\nue\nueb}\xspace}
\def\num        {\ensuremath{\nu_\mu}\xspace}
\def\numb       {\ensuremath{\nub_\mu}\xspace}
\def\numnumb    {\ensuremath{\num\numb}\xspace}
\def\nut        {\ensuremath{\nu_\tau}\xspace}
\def\nutb       {\ensuremath{\nub_\tau}\xspace}
\def\nutnutb    {\ensuremath{\nut\nutb}\xspace}
\def\nul        {\ensuremath{\nu_\ell}\xspace}
\def\nulb       {\ensuremath{\nub_\ell}\xspace}
\def\nulnulb    {\ensuremath{\nul\nulb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {\ensuremath{\gamma}\xspace}
\def\gaga  {\ensuremath{\gamma\gamma}\xspace}  %% changed from \gg, which is >>
\def\ggstar{\ensuremath{\gamma\gamma^*}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  LEPTONS, PHOTONS and other GAUGE BOSONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ega   {\ensuremath{e\gamma}\xspace}
\def\game  {\ensuremath{\gamma e^-}\xspace}
\def\epemg  {\ensuremath{e^+e^-\gamma}\xspace}
\def\H  {\ensuremath{H^0}\xspace}
\def\Hp     {\ensuremath{H^+}\xspace}
\def\Hm     {\ensuremath{H^-}\xspace}
\def\Hpm    {\ensuremath{H^\pm}\xspace}
\def\W      {\ensuremath{W}\xspace}
\def\Wp     {\ensuremath{W^+}\xspace}
\def\Wm     {\ensuremath{W^-}\xspace}
\def\Wpm    {\ensuremath{W^\pm}\xspace}
\def\Z      {\ensuremath{Z^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q   {\ensuremath{q}\xspace}
\def\qbar  {\ensuremath{\overline q}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}
\def\u  {\ensuremath{u}\xspace}
\def\ubar  {\ensuremath{\overline u}\xspace}
\def\uubar {\ensuremath{u\overline u}\xspace}
\def\d  {\ensuremath{d}\xspace}
\def\dbar  {\ensuremath{\overline d}\xspace}
\def\ddbar {\ensuremath{d\overline d}\xspace}
\def\s  {\ensuremath{s}\xspace}
\def\sbar  {\ensuremath{\overline s}\xspace}
\def\ssbar {\ensuremath{s\overline s}\xspace}
\def\c  {\ensuremath{c}\xspace}
\def\cbar  {\ensuremath{\overline c}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}
\def\b  {\ensuremath{b}\xspace}
\def\bbar  {\ensuremath{\overline b}\xspace}
\def\bbbar {\ensuremath{b\overline b}\xspace}
\def\t  {\ensuremath{t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\ttbar {\ensuremath{t\overline t}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   HADRONS   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pizs  {\ensuremath{\pi^0\mbox\,\rm{s}}\xspace}
\def\ppz   {\ensuremath{\pi^0\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\pipi  {\ensuremath{\pi^+\pi^-}\xspace}
\def\pipm   {\ensuremath{\pi^\pm}\xspace}
\def\pimp   {\ensuremath{\pi^\mp}\xspace}
\def\kaon  {\ensuremath{K}\xspace}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}\xspace}
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kpm   {\ensuremath{K^\pm}\xspace}
\def\Kmp   {\ensuremath{K^\mp}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace} 
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}\xspace} 
\def\Kstarz  {\ensuremath{K^{*0}}\xspace}
\def\Kstarzb  {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{K^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp   {\ensuremath{K^{*+}}\xspace}
\def\Kstarm   {\ensuremath{K^{*-}}\xspace}
\def\Kstarpm   {\ensuremath{K^{*\pm}}\xspace}
\def\Kstarmp   {\ensuremath{K^{*\mp}}\xspace}
\def\Kz   {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{K^0 \kern -0.16em \Kzb}\xspace}
\def\Dz    {\ensuremath{D^0}\xspace}
\def\Dpm    {\ensuremath{D^\pm}\xspace}
%%% do NOT use ensuremath here
\def\Dbar  {\kern 0.2em\overline{\kern -0.2em D}{}\xspace}
\def\Db    {\ensuremath{\Dbar}\xspace}
\def\Dzb   {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb {\ensuremath{D^0 {\kern -0.16em \Dzb}}\xspace}
\def\Dstar   {\ensuremath{D^*}\xspace}
\def\Dstarb   {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{D^{*0}}\xspace}
\def\Dstarzb  {\ensuremath{\Dbar^{*0}}\xspace}
\def\Ds    {\ensuremath{D^+_s}\xspace}
\def\Dsb   {\ensuremath{\Dbar^+_s}\xspace}
\def\Dss   {\ensuremath{D^*_s}\xspace}
\def\Bz    {\ensuremath{B^0}\xspace}
\def\B     {\ensuremath{B}\xspace}
%%% do NOT use ensuremath here
\def\Bbar  {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb    {\ensuremath{\Bbar}\xspace}
\def\Bzb   {\ensuremath{\Bbar^0}\xspace}
\def\Bu    {\ensuremath{B^+}\xspace}
\def\Bub   {\ensuremath{B^-}\xspace}
\def\Bpm   {\ensuremath{B^\pm}\xspace}
\def\Bmp   {\ensuremath{B^\mp}\xspace}
\def\Bs    {\ensuremath{B_s}\xspace}
\def\Bsb   {\ensuremath{\Bbar_s}\xspace}
\def\BB    {\ensuremath{B\Bbar}\xspace} 
\def\BzBzb {\ensuremath{B^0 {\kern -0.16em \Bzb}}\xspace}
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}\xspace}

\def\jpsi  {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\psitwos {\ensuremath{\psi{(2S)}}\xspace}
\def\psiprpr {\ensuremath{\psi(3770)}\xspace}
\def\etac    {\ensuremath{\eta_c}\xspace}
\def\chiczero {\ensuremath{\chi_{c0}}\xspace}
\def\chicone {\ensuremath{\chi_{c1}}\xspace}
\def\chictwo {\ensuremath{\chi_{c2}}\xspace}
\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}
\def\X {\ensuremath{X}}

\def\proton     {\ensuremath{p}\xspace}
\def\antiproton {\ensuremath{\overline p}\xspace}
\def\neutron    {\ensuremath{n}\xspace}
\def\antineutron  {\ensuremath{\overline n}\xspace}

\mathchardef\Deltares="7101
\mathchardef\Xi="7104
\mathchardef\Lambda="7103
\mathchardef\Sigma="7106
\mathchardef\Omega="710A
%%% do NOT use ensuremath here
\def\Deltabar   {\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
\def\Lbar {\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
\def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
\def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  BRANCHING RATIOS %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\BR{{\ensuremath{\cal B}}}
\def\BRtauptoe  {\ensuremath{\BR(\taup \to \ep)}}
\def\BRtaumtoe  {\ensuremath{\BR(\taum \to \en)}}
\def\BRtauptomu {\ensuremath{\BR(\taup \to \mup)}}
\def\BRtaumtomu {\ensuremath{\BR(\taum \to \mun)}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  REACTIONS    %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\upsbb {\ensuremath{\Upsilon{\rm( 4S)}\to B\Bbar}} 
\def\upsbzbz {\ensuremath{\Upsilon{\rm( 4S)}\to\BzBzb}} 
\def\upsbpbm {\ensuremath{\Upsilon{\rm( 4S)}\to\Bu\Bub}} 
\def\bpsiks{\ensuremath{B^0 \to \jpsi \KS}}
\def\bpsikst{\ensuremath{B^0 \to \jpsi \Kstar}}
\def\bpsikl{\ensuremath{B^0 \to \jpsi \KL}}
\def\bpsikzeropi{\ensuremath{B^0 \to \jpsi (K^{*0} \to \KL\pi^0)}}
\def\bpsikpluspi{\ensuremath{B^+ \to \jpsi K^{*+},\ K^{*+} \to \KL\pi^+}}
\def\bpsikpluspi{\ensuremath{
{\Bz}/B^0 \to \jpsi ( \to \mu^+ \mu^-) K^{\pm} \pi^{\mp} }}
\def\bupsik{\ensuremath{B^{\pm} \to \jpsi ( \to \mu^+ \mu^-) K^{\pm} }}
\def\bpsiX{\ensuremath{B^0 \to \jpsi X}}
\def\upspsikl{\ensuremath{\FourS\to (\bpsikl) (\bzb \to X)}}
\def\Bzbtomu    {\ensuremath{\Bzb \to \mu {\rm X}}}
\def\Bzbtox     {\ensuremath{\Bzb \to {\rm X}}}
\def\Bztopipi   {\ensuremath{B^0 \to \pipi}}
\def\Bztokpi    {\ensuremath{B^0 \to K^{\pm}\pi^{\mp}}}
\def\Bztorhopi  {\ensuremath{B^0 \to \rho^+\pi^-}}
\def\Bztorhorho {\ensuremath{B^0 \to \rho\rho}}
\def\Bztokrho   {\ensuremath{B^0 \to K\rho}}
\def\Bztokstpi  {\ensuremath{B^0 \to \Kstar\pi}}
\def\Bztoapi    {\ensuremath{B^0 \to a_1\pi}}
\def\Bztodd     {\ensuremath{B^0 \to D^+D^-}}
\def\Bztodstd   {\ensuremath{B^0 \to D^{*+}D^-}}
\def\Bztodstdst {\ensuremath{B^0 \to D^{*+}D^{*-}}}
\def\BtoDK      {\ensuremath{B \to DK}}
\def\Btodstlnu  {\ensuremath{B \to D^*l\nu}}
\def\Btodstdlnu {\ensuremath{B \to D^*(D)l\nu}}
\def\Btorholnu  {\ensuremath{B \to \rho l\nu}}
\def\Btopilnu   {\ensuremath{B \to \pi l\nu}}
\def\Btoetah    {\ensuremath{B \to \eta h}}
\def\Btoetaph   {\ensuremath{B \to \eta ' h}}
\def\tauptoe    {\ensuremath{\taup \to \ep \nu \overline \nu}}
\def\taumtoe    {\ensuremath{\taum \to \en \nu \overline \nu}}
\def\tauptomu   {\ensuremath{\taup \to \mup \nu \overline \nu}}
\def\taumtomu    {\ensuremath{\taum \to \mun \nu \overline \nu}}
\def\Btoetaph   {\ensuremath{B \to \eta ' h}}
\def\tauptopi   {\ensuremath{\taup \to \pip \overline \nu}}
\def\taumtopi   {\ensuremath{\taum \to \pim \nu}}
\def\ggtopi     {\ensuremath{\gaga \to \pipi}}
\def\ggtopiz    {\ensuremath{\gaga \to \ppz}}
\def\ggstox     {\ensuremath{\ggstar \to \X(1420) \to \kaon \kaon \pi}}
\def\ggstoeta   {\ensuremath{\ggstar \to \eta(550) \to \pipi \piz}}
\def\btosgam   {\ensuremath{b \to s \gamma}}
\def\btodgam   {\ensuremath{b \to d \gamma}}
\def\btosll    {\ensuremath{b \to s l^+l^-}}
\def\btosnunu   {\ensuremath{b \to s \nu\nub}}
\def\btosgaga   {\ensuremath{b \to s \gaga}}
\def\btosglue   {\ensuremath{b \to s g}}


% Kinematics

\def\ptot       {\mbox{$p$}\xspace}
%\def\pxy        {\mbox{$p_{\rm t}$}
\def\pxy        {\mbox{$p_T$}\xspace}
%\def\pt         {\mbox{$p_{\rm t}$}\xspace}
\def\pt         {\mbox{$p_T$}\xspace}
\def\mes        {\mbox{$m_{\rm ES}$}\xspace}
\def\mec        {\mbox{$m_{\rm EC}$}\xspace}


% Geometry
\def\mphi       {\mbox{$\phi$}\xspace}
\def\mtheta     {\mbox{$\theta$}\xspace}
\def\ctheta     {\mbox{$\cos \theta$}\xspace}

% UNITS
%
\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}
%\def\ev   {\ensuremath{\rm \,e\kern -0.08em V}}
%\def\kev  {\ensuremath{\rm \,ke\kern -0.08em V}} 
%\def\mev  {\ensuremath{\rm \,Me\kern -0.08em V}} 
%\def\gev  {\ensuremath{\rm \,Ge\kern -0.08em V}} 
%\def\gevc {\ensuremath{\rm \,Ge\kern -0.08em V\!/c}} 
%\def\gevc {\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c}} 
%\def\tev  {\ensuremath{\rm \,Te\kern -0.08em V}}
%\def\mevc {\ensuremath{\rm \,Me\kern -0.08em V\!/c}} 
%\def\mevc {\ensuremath{{\rm \,Me\kern -0.08em V\!/}c}} 
%\def\gevcc{\ensuremath{\rm \,Ge\kern -0.08em V\!/c^2}} 
%\def\mevcc{\ensuremath{\rm \,Me\kern -0.08em V\!/c^2}} 
%\def\gevcc{\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c^2}} 
%\def\mevcc{\ensuremath{{\rm \,Me\kern -0.08em V\!/}c^2}} 
\def\syin {\ensuremath{^{\prime\prime}}\xspace}
\def\inch   {\ensuremath{\rm \,in}\xspace} % \in is taken
\def\ft   {\ensuremath{\rm \,ft}\xspace}
\def\km   {\ensuremath{\rm \,km}\xspace}
\def\m    {\ensuremath{\rm \,m}\xspace}
\def\cm   {\ensuremath{\rm \,cm}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mm   {\ensuremath{\rm \,mm}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
%\def\mum  {\ensuremath{\rm \,\mum}\xspace}
\def\mum  {\ensuremath{\,\mu\rm m}\xspace}%% mu meter 
%\def\muma {\ensuremath{\rm \,\mum}^2\xspace}
\def\muma       {\ensuremath{\,\mu\rm m^2}\xspace}
\def\nm   {\ensuremath{\rm \,nm}\xspace}
\def\fm   {\ensuremath{\rm \,fm}\xspace}
%
\def\barn{\ensuremath{\rm \,b}\xspace}
\def\barnhyph{\ensuremath{\rm -b}\xspace}
\def\mbarn{\ensuremath{\rm \,mb}\xspace}
\def\mbarnhyph{\ensuremath{\rm -mb}\xspace}
\def\pb {\ensuremath{\rm \,pb}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
%
\def\mus  {\ensuremath{\rm \,\mus}\xspace}
\def\ns   {\ensuremath{\rm \,ns}\xspace}
\def\ps   {\ensuremath{\rm \,ps}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}
\def\gm   {\ensuremath{\rm \,g}\xspace}
%
\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\let\dgr\degrees

%
% Lengths / Areas
%
%\def\m          {\ensuremath{\rm \,m}}    %% meter
%\def\ma         {\ensuremath{\rm \,m}^2}  %% meter squared
%\def\cm         {\ensuremath{\rm \,cm}}   %% centimeter
%\def\cma        {\ensuremath{\rm \,cm}^2} %% centimeter squared
%\def\cms         {\ensuremath{{\rm \,cm}^{-2} {\rm s}^{-1}}\xspace}
%\def\mm         {\ensuremath{\rm \,mm}}   %% millimeter
%\def\mma        {\ensuremath{\rm \,mm}^2} %% millimeter squared
%\def\mum        {\ensuremath{\,\mu\rm m}} %% mu meter
%\def\muma       {\ensuremath{\,\mu\rm m^2}}
%
\def\nm         {\ensuremath{\rm \,nm}\xspace}   %% nanometer
\def\nb         {\ensuremath{\rm \,nb}\xspace}
%%%%%
% Time
%%\def\s{\ensuremath{\rm {\,s}}} %% second - this displays nothing  - why?
\def\sec{\ensuremath{\rm {\,s}}\xspace}       %% second - this works - jw 4/19
\def\ms         {\ensuremath{{\rm \,ms}}\xspace}     %% millisecond
\def\mus        {\ensuremath{\,\mu{\rm s}}\xspace}    %% microsecond
\def\ns         {\ensuremath{{\rm \,ns}}\xspace}      %% nanosecond
\def\ps         {\ensuremath{{\rm \,ps}}\xspace}  %% picosecond
%
% Data processing
\def\kbytes     {\ensuremath{{\rm \,kbytes}}\xspace}
\def\kbsps      {\ensuremath{{\rm \,kbytes/s}}\xspace}
\def\kbits      {\ensuremath{{\rm \,kbits}}\xspace}
\def\kbsps      {\ensuremath{{\rm \,kbits/s}}\xspace}
\def\mbsps      {\ensuremath{{\rm \,Mbits/s}}\xspace}
\def\mbytes     {\ensuremath{{\rm \,Mbytes}}\xspace}
\def\mbps       {\ensuremath{{\rm \,Mbyte/s}}\xspace}
\def\mbsps      {\ensuremath{{\rm \,Mbytes/s}}\xspace}
\def\gbsps      {\ensuremath{{\rm \,Gbits/s}}\xspace}
\def\gbytes     {\ensuremath{{\rm \,Gbytes}}\xspace}
\def\gbsps      {\ensuremath{{\rm \,Gbytes/s}}\xspace}
\def\tbytes     {\ensuremath{{\rm \,Tbytes}}\xspace}
\def\tbpy       {\ensuremath{{\rm \,Tbytes/yr}}\xspace}
%

\def\mic  {\ensuremath{\,\mu{\rm C}}\xspace}
\def\krad {\ensuremath{\rm \,krad}\xspace}
\def\cmc  {\ensuremath{{\rm \,cm}^3}\xspace}
\def\yr   {\ensuremath{\rm \,yr}\xspace}
\def\hr   {\ensuremath{\rm \,hr}\xspace}
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\rm K}\xspace}
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\mrad{\ensuremath{\rm \,mr}\xspace}               %% milliradian
\def\mradhyph{\ensuremath{\rm -mr}\xspace}
%
\def\sx    {\ensuremath{\sigma_x}\xspace}    
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}    

%\renewcommand{\bar}[1]{\overline{#1}}  

% Some more (from Helen)
%\def\O{{\ensuremath{\cal O}}}  !!! This is a predefined LaTeX symbol !!!
\def\order{{\ensuremath{\cal O}}\xspace}
\def\L{{\ensuremath{\cal L}}\xspace}
\def\calL{{\ensuremath{\cal L}}\xspace}
%\def\S{{\ensuremath{\cal S}}}  !!! This is a predefined LaTeX symbol !!!
\def\calS{{\ensuremath{\cal S}}\xspace}
\def\calA{{\ensuremath{\cal A}}\xspace}
\def\calD{{\ensuremath{\cal D}}\xspace}
\def\calR{{\ensuremath{\cal R}}\xspace}
\def\eps{\varepsilon\xspace}
\def\epsK{\varepsilon_K\xspace}
\def\epsB{\varepsilon_B\xspace}
\def\epsp{\varepsilon^\prime_K\xspace}
\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\qsq                {\ensuremath{q^2}\xspace}
\def\CP                 {\ensuremath{C\!P}\xspace}
%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}
\def\epstag  {\ensuremath{\epsilon_{\rm tag}}\xspace}
\def\tagfac  {\ensuremath{\epstag(1-2w)^2}\xspace}
\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}}
\newcommand{\syst}{\ensuremath{\mathrm{(syst)}}}

% Common combinations
\def\pep2{PEP-II}
\def\BF{$B$ Factory}
\def\abf {asymmetric \BF}
\def\sx    {\ensuremath{\sigma_x}\xspace}     
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}

\def\pbcm {\ensuremath{p^*_{B^0}}\xspace}
%\def\chic1{\ensuremath{\chi_{c1}}}
%\def\chic2{\ensuremath{\chi_{c2}}}
%\def\chic3{\ensuremath{\chi_{c3}}}
\def\chic#1{\ensuremath{\chi_{c#1}}\xspace} % dbm

\newcommand{\etapr}{\ensuremath{\eta^{\prime}}\xspace}
\newcommand{\Betaprks}{\ensuremath{\bz\ra\etapr\KS}\xspace}
\newcommand{\Betaprkz}{\ensuremath{\bz\ra\etapr K^0}\xspace}
\newcommand{\etaprepp}{\ensuremath{\etapr\ra\eta\pipi}\xspace}
\newcommand{\etaprrg}{\ensuremath{\etapr\ra\rho^0\gamma}\xspace}

\newcommand{\inverse}{\ensuremath{^{-1}}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\delm}{\ensuremath{m_{\dstr}-m_{\dz}}\xspace}

\newcommand{\dstr}{\ensuremath{D^{*}}\xspace}
\newcommand{\dstrstr}{\ensuremath{D^{**}}\xspace}
\newcommand{\dsp}{\ensuremath{D^{*+}}\xspace}
\newcommand{\dsm}{\ensuremath{D^{*-}}\xspace}
\newcommand{\dsz}{\ensuremath{D^{*0}}\xspace}
 
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}

% QCD parameters

\newcommand{\as}{\ensuremath{\alpha_{\scriptscriptstyle S}}\xspace}
\newcommand{\MSb}{\ensuremath{\overline{\mathrm{MS}}}\xspace}
\newcommand{\LMSb}{%
  \ensuremath{\Lambda_{\overline{\scriptscriptstyle\mathrm{MS}}}}\xspace
}

% Electroweak parameters

\newcommand{\tw}{\ensuremath{\theta_{\scriptscriptstyle W}}\xspace}
\newcommand{\twb}{%
  \ensuremath{\overline{\theta}_{\scriptscriptstyle W}}\xspace
}
\newcommand{\Afb}[1]{{\ensuremath{A_{\scriptscriptstyle FB}^{#1}}}}
\newcommand{\gv}[1]{{\ensuremath{g_{\scriptscriptstyle V}^{#1}}}}
\newcommand{\ga}[1]{{\ensuremath{g_{\scriptscriptstyle A}^{#1}}}}
\newcommand{\gvb}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle V}^{#1}}}}
\newcommand{\gab}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle A}^{#1}}}}


\def\rhobar {\ensuremath{\overline \rho}\xspace}
\def\etabar {\ensuremath{\overline \eta}\xspace}
%\def\paramest {\ensuremath{{\hat A}, {\hat \rho}, {\hat \eta} }}
%\def\ssparamest {\ensuremath{{\hat A}, {\hat {\sin 2 \alpha}}, 
%{\hat {\sin 2 \beta}} }}
\def\meas {\ensuremath{|V_{cb}|, |\frac{V_{ub}}{V_{cb}}|, 
|\varepsilon_K|, \Delta m_{B_d}}\xspace}

\def\Vud  {\ensuremath{|V_{ud}|}\xspace}
\def\Vcd  {\ensuremath{|V_{cd}|}\xspace}
\def\Vtd  {\ensuremath{|V_{td}|}\xspace}
\def\Vus  {\ensuremath{|V_{us}|}\xspace}
\def\Vcs  {\ensuremath{|V_{cs}|}\xspace}
\def\Vts  {\ensuremath{|V_{ts}|}\xspace}
\def\Vub  {\ensuremath{|V_{ub}|}\xspace}
\def\Vcb  {\ensuremath{|V_{cb}|}\xspace}
\def\Vtb  {\ensuremath{|V_{tb}|}\xspace}

%\def\sa{${\sin\! 2 \alpha  }$\xspace}
%\def\sb{${\sin\! 2 \beta   }$\xspace}
%\def\sg{${\sin\! 2 \gamma  }$\xspace}

% added by Gautier for tagging, tagmix, and sin2beta
\def\stwoa{\ensuremath{\sin\! 2 \alpha  }\xspace}
\def\stwob{\ensuremath{\sin\! 2 \beta   }\xspace}
\def\stwog{\ensuremath{\sin\! 2 \gamma  }\xspace}
\def\mistag{\ensuremath{w}\xspace}
\def\dilution{\ensuremath{\cal D}\xspace}
\def\deltaz{\ensuremath{{\rm \Delta}z}\xspace}
\def\deltat{\ensuremath{{\rm \Delta}t}\xspace}
\def\deltamd{\ensuremath{{\rm \Delta}m_d}\xspace}

\newcommand{\fsubd}{\ensuremath{f_D}}\xspace
\newcommand{\fds}{\ensuremath{f_{D_s}}\xspace}
\newcommand{\fsubb}{\ensuremath{f_B}\xspace}
\newcommand{\fbd}{\ensuremath{f_{B_d}}\xspace}
\newcommand{\fbs}{\ensuremath{f_{B_s}}\xspace}
\newcommand{\bsubb}{\ensuremath{B_B}\xspace}
\newcommand{\bbd}{\ensuremath{B_{B_d}}\xspace}
\newcommand{\bbs}{\ensuremath{B_{B_s}}\xspace}
\newcommand{\rgbb}{\ensuremath{\hat{B}_B}\xspace}
\newcommand{\rgbbd}{\ensuremath{\hat{B}_{B_d}}\xspace}
\newcommand{\rgbbs}{\ensuremath{\hat{B}_{B_s}}\xspace}
\newcommand{\rgbk}{\ensuremath{\hat{B}_K}\xspace}
\newcommand{\lqcd}{\ensuremath{\Lambda_{\mathrm{QCD}}}\xspace}

%\newcommand{\eqref}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\subsecref}[1]{Section~\ref{subsec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}






% Journal References
\newcommand{\ace}       [1]  {{Adv.\ Cry.\ Eng.\ {\bf #1}}}
\newcommand{\arnps}     [1]  {{Ann.\ Rev.\ Nucl.\ Part.\ Sci.\ {\bf #1}}}
\newcommand{\arns}      [1]  {{Ann.\ Rev.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\appopt}    [1]  {{Appl.\ Opt.\ {\bf #1}}}
\newcommand{\seis}      [1]  {{Bull.\ Seismological Soc.\ of Am.\ {\bf #1}}}
\newcommand{\epjc}      [1]  {{Eur.\ Phys.\ Jour.\ C~{\bf #1}}}
\newcommand{\ited}      [1]  {{IEEE Trans.\ Electron.\ Devices~{\bf #1}}}
\newcommand{\itns}      [1]  {{IEEE Trans.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\ijqe}      [1]  {{IEEE J.\ Quantum Electron.\ {\bf #1}}}
\newcommand{\ijmp}      [1]  {{Int.\ Jour.\ Mod.\ Phys.\ {\bf #1}}}
\newcommand{\ijmpa}     [1]  {{Int.\ J.\ Mod.\ Phys.\ {\bf A{\bf #1}}}}
\newcommand{\jl}        [1]  {{JETP Lett.\ {\bf #1}}}
\newcommand{\jetp}      [1]  {{JETP~{\bf #1}}}
\newcommand{\jpg}       [1]  {{J.\ Phys.\ {G{\bf #1}}}}
\newcommand{\jap}       [1]  {{J.\ Appl.\ Phys.\ {\bf #1}}}
\newcommand{\jmp}       [1]  {{J.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\jmes}      [1]  {{J.\ Micro.\ Elec.\ Sys.\ {\bf #1}}}
%\newcommand{\josa}      [1]  {{J.\ Opt.\ Soc.\ Am.\ {\bf #1}}}
\newcommand{\nim}       [1]  {{Nucl.\ Instr.\ and Methods~{\bf #1}}}
\newcommand{\nima}      [1]  {{Nucl.\ Instr.\ Methods {A{\bf #1}}}}
\newcommand{\np}        [1]  {{Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\npb}       [1]  {{Nucl.\ Phys.\ {\bf B{\bf #1}}}}
\newcommand{\npps}      [1]  {{Nucl.\ Phys.\ Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\npp}      [1]  {{Nucl.\ Phys.\ Proc.\ {\bf #1}}}
\newcommand{\npbps}     [1]  {{Nucl.\ Phys.\ B Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\ncim}      [1]  {{Nuo.\ Cim.\ {\bf #1}}}
\newcommand{\optl}      [1]  {{Opt.\ Lett.\ {\bf #1}}}
\newcommand{\optcom}    [1]  {{Opt.\ Commun.\ {\bf #1}}}
\newcommand{\partacc}   [1]  {{Particle Acclerators~{\bf #1}}}
\newcommand{\pflu}      [1]  {{Physics of Fluids~{\bf #1}}}
\newcommand{\ptoday}    [1]  {{Physics Today~{\bf #1}}}
\newcommand{\jpl}        [1]  {{Phys.\ Lett.\ {\bf #1}}}      % dbm
\newcommand{\plb}       [1]  {{Phys.\ Lett.\ B~{\bf #1}}}   % dbm
\newcommand{\prep}      [1]  {{Phys.\ Rep.{\bf #1}}}
\newcommand{\jprl}       [1]  {{Phys.\ Rev.\ Lett.\ {\bf #1}}} % dbm
\newcommand{\pr}        [1]  {{Phys.\ Rev.\ {\bf #1}}}
\newcommand{\jpra}       [1]  {{Phys.\ Rev.\ A~{\bf #1}}}
\newcommand{\jprd}       [1]  {{Phys.\ Rev.\ D~{\bf #1}}}
\newcommand{\jpre}       [1]  {{Phys.\ Rev.\ E~{\bf #1}}}
\newcommand{\progtp}    [1]  {{Prog.\ Th.\ Phys.\ {\bf #1}}}
\newcommand{\jrmp}       [1]  {{Rev.\ Mod.\ Phys.\ {\bf #1}}}  % dbm
\newcommand{\rsi}       [1]  {{Rev.\ Sci.\ Instr.\ {\bf #1}}}
\newcommand{\sci}       [1]  {{Science~{\bf #1}}}
\newcommand{\sjnp}      [1]  {{Sov.\ J.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\spu}       [1]  {{Sov.\ Phys.\ Usp.\ {\bf #1}}}
\newcommand{\tmf}       [1]  {{Teor.\ Mat.\ Fiz.\ {\bf #1}}}
\newcommand{\yf}        [1]  {{Yad.\ Fiz.\ {\bf #1}}}
\newcommand{\zpc}       [1]  {{Z.\ Phys.\ C~{\bf #1}}}
%\newcommand{\zp}        [1]  {{Z.\ Phys.\ {\bf #1}}}
\newcommand{\zpr}       [1]  {{ZhETF Pis.\ Red.\ {\bf #1}}}
\newcommand{\cpc}   [1]  {{Comput.\ Phys.\ Commun.\ {\bf #1}}}
\newcommand{\mpl}     [1]  {{Mod.\ Phys.\ Lett.\ {\bf #1}}}
\newcommand{\fp}       [1]   {{Fortschr.\ Phys.\ {\bf #1}}}
\newcommand{\cnpp}  [1]   {{Comm.\ Nucl.\ Part.\ Phys.\ {\bf #1}}}
\newcommand{\rpp}   [1]    {{Rep.\ Prog.\ Phys.\ {\bf #1}}}
\newcommand{\app}  [1]    {{Acta Phys.\ Polon.\ {\bf #1}}}
\newcommand{\fizika}[1]   {{Fizika~{\bf #1}}}
\newcommand{\spd}  [1]    {{Sov.\ Phys.\ Dokl.\ {\bf #1}}}
\newcommand{\baps} [1]  {{Bull.\ Am.\ Phys.\ Soc.\ {\bf #1}}}
\newcommand{\araa} [1]   {{Ann.\ Rev.\ Astr.\ Ap.\ {\bf #1}}}
\newcommand{\japj} [1]     {{Astro.\ Phys.\ J.\ {\bf #1}}}
\newcommand{\annp}  [1]  {{Ann.\ Phys.\ {\bf #1}}}
\newcommand{\ppnp}  [1]  {{Prog.\ Part.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\prsl}  [1]    {{Proc.\ Roy.\ Soc.\ Lond.\ {\bf #1}}}
\newcommand{\apas}  [1]  {{Acta Phys.\ Austr.\ Suppl.\ {\bf #1}}}
\newcommand{\anp}  [1]  {{Adv.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\pan}  [1]  {{Phys.\ Atom.\ Nuclei~{\bf #1}}}
\newcommand{\cmp} [1]  {{Commun.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\npaps} [1]  {{Nucl.\ Phys.\ A (Proc.\ Suppl.)~{\bf #1}}}

%%%%%%%%%%%%%%%%%%%% SOFTWARE PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\aslund     {\mbox{\tt Aslund}}
\def\bbsim      {\mbox{\tt BBsim}}
\def\beast      {\mbox{\tt Beast}}
\def\beget      {\mbox{\tt Beget}}
\def\Bta        {\mbox{\tt Beta}}
\def\betakfit   {\mbox{\tt BetaKfit}}
\def\cornelius  {\mbox{\tt Cornelius}}
\def\evtgen     {\mbox{\tt EvtGen}}
\def\euclid     {\mbox{\tt Euclid}}
\def\fitver     {\mbox{\tt FitVer}}
\def\fluka      {\mbox{\tt Fluka}}
\def\fortran    {\mbox{\tt Fortran}}
\def\gcalor     {\mbox{\tt GCalor}}
\def\geant      {\mbox{\tt GEANT}}%
\def\gheisha    {\mbox{\tt Gheisha}}
\def\jetset74   {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}}
%\def\jetset    {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}}
\def\koralb     {\mbox{\tt KoralB}}
\def\minuit     {\mbox{\tt Minuit}}
\def\objegs     {\mbox{\tt Objegs}}
\def\turtle     {\mbox{\tt Decay~Turtle}}
\def\hemicosm   {\mbox{\tt HemiCosm}}
\def\stdhep     {\mbox{\tt StdHep}}
\def\hepevt     {\mbox{\tt{/HepEvt/}}}
\def\squaw      {\mbox{\tt Squaw}}
\def\trackerr   {\mbox{\tt TrackErr}}


==> interpretation.tex <==


In a second stage, we transform the combined $(\xbpmtrue,\ybpmtrue)$, $(\xbstpmtrue,\ybstpmtrue)$, and $(\xspmtrue,\yspmtrue)$
measurements into 
the physically relevant quantities \g and the set of hadronic parameters
$\uvec \equiv (\rb, \rbst, \krs, \deltab, \deltabst, \deltas)$.
We adopt a
frequentist procedure~\cite{ref:woodroofe} to obtain one-dimensional confidence intervals
of well-defined \CL that takes into account
non-Gaussian effects due to the nonlinearity of the relations between the observables and physical quantities.
This procedure is identical to that used in Refs.~\cite{ref:GGSZ2008,ref:GGSZ2010,ref:GLW_d0k,ref:GLWADS_d0kstar,ref:ADS_d0k_dstar0k_kpi}.

We define a $\chi^2$ function as 
\begin{eqnarray}
\chi^2(\g, \uvec) &\equiv& -\twoDLL(\g,\uvec)\nn\\
 &\equiv& -2 [ \ln{\cal L}(\g,\uvec) - \ln{\cal L}_{\mathrm{max}} ],~
\end{eqnarray}
where $\twoDLL(\g,\uvec)$ is the variation of the combined
log-likelihood with respect to its maximum value,
with the \zbzbstpmtrue and \zspmtrue expected values written in terms
of \g and \uvec, i.e., replacing \zbzbstpmtrue and \zspmtrue by $\rbrbst e^{i(\deltabdeltabst \pm \g)}$ 
and $\kappa \rs e^{i(\deltas \pm \g)}$, respectively.
To evaluate the \CL of a certain parameter (for example \g) at a given value ($\g_0$), we consider the value of 
the $\chi^2$ function at the new minimum, $\chi^2_\mathrm{min}(\g_0,\uvec_0)$, satisfying $\Delta \chi^2(\g_0) = \chi^2_\mathrm{min}(\g_0,\uvec_0) - \chi^2_\mathrm{min} \ge 0$.
In a purely Gaussian situation, 
the \CL is given by the probability that $\Delta \chi^2(\g_0)$ is exceeded for 
a $\chi^2$ distribution with one degree of freedom, $1-\CL = {\mathrm Prob}[\Delta \chi^2(\g_0);\nu=1]$, where $\mathrm{Prob}[\Delta \chi^2(\g_0);\nu=1]$ is 
the corresponding cumulative distribution function (this approach is later referred to as ``Prob method'')~\cite{ref:pdg2010}. 
In a non-Gaussian situation one has to consider $\Delta \chi^2(\gamma_0)$ as a test statistic, and 
rely on a Monte Carlo simulation to obtain its expected distribution. 
This Monte Carlo simulation is performed by
generating 
more than $10^9$ samples 
(sets of the 39 GGSZ, GLW, ADS, and \D decay observable values), using the combined likelihood 
evaluated at values $(\g_0,\uvec_0)$, i.e., ${\cal L}(\g_0,\uvec_0)$.
The confidence level $\CL$ is determined from the fraction of experiments for which
$\Delta \chi'^2(\g_0) > \Delta \chi^2(\g_0)$,
where $\Delta \chi'^2(\g_0) = \chi'^2(\g_0,\uvec'_0) - \chi'^2_{\mathrm{min}}$ for each simulated experiment 
is determined as in the case of the actual data sample. 
We allow $0 \le \rbrbst,\krs \le 1$ and $-180^\circ \le \g, \deltabdeltabst,\deltas \le 180^\circ$.

Figure~\ref{fig:scans-gamma-rb-delta} illustrates $1-\CL$ as a function of \g, \rbrbst, \krs, \deltabdeltabst, and \deltas,
for each of the three \B decay channels separately and, in the case of \g, their combination.
The combination has the same twofold ambiguity in the weak and strong phases
as that of the GGSZ method,
$(\gamma;\deltabdeltabst,\deltas) \to (\gamma + 180^\circ; \deltabdeltabst + 180^\circ,\deltas+180^\circ)$.
From these distributions, we extract one- and two-standard-deviation intervals as the sets of values for which
$1-\CL$ is greater than 31.73\% and 4.55\%, respectively, as summarized in Table~\ref{tab:polarresults}.
When comparing these intervals to those obtained with the GGSZ method only, also shown in Table~\ref{tab:polarresults},
we observe that the combination helps improving the constraints on \rbrbst and \krs, but not those on \g.
To assess the impact of the GLW and ADS observables in the determination of \g, we compare $1-\CL$ as a function of \rbrbst and \g 
for all \B decay channels combined using the GGSZ method alone, the combination with the GLW measurements, and the global combination, 
as shown in Fig.~\ref{fig:scan-comp-rb+gamma}. While the constraints on \rb are clearly 
improved at the one- and two-standard-deviation level, and to a lesser extent on \rbst, their best (central) values move towards slightly
lower values. Since the uncertainty on \g scales approximately as $1/\rbrbst$,
the constraints on \g at $68.3\%$ and $95.4\%$ \CL do not improve,
in spite of the tighter constraints on the combined measurements shown in Fig.~\ref{fig:xyresults}.
However, adding GLW and ADS information reduces the confidence intervals for smaller $1-\CL$, as a consequence of
the more Gaussian behavior when the significance of excluding $\rbrbst=0$ increases.
Thus, for example, in the region close to four standard deviations, the GGSZ method alone 
does not constrain \g, while the combination is able to exclude large regions.

\begin{figure}[htb!]
\begin{center}
\epsfig{file=scan-gammat-DalitzGLWADSRPMHIST.eps,width=0.85\linewidth} \\
\epsfig{file=scan-rbt-DalitzGLWADSRPMHIST.eps,width=0.85\linewidth} \\
\epsfig{file=scan-deltat-DalitzGLWADSRPMHIST.eps,width=0.85\linewidth}
\end{center}
\caption{(color online). 
$1-\CL$ distributions for the combination of the GGSZ, GLW and ADS methods
as a function of \g (top), \rbrbst, and \krs (middle), and \deltabdeltabst, \deltas (bottom),
including statistical and systematic uncertainties,
for $\Bpm \to \D \Kpm$, $\Bpm \to \Dstar \Kpm$, and $\Bpm \to \D \Kstarpm$ decays. The combination of all the \B decay channels is also shown for \g.
The dashed (dotted) horizontal line corresponds to the one- (two-) standard-deviation \CL.
\label{fig:scans-gamma-rb-delta}
}
\end{figure}
%
%
%
\begin{figure}[htb!]
\begin{center}
\begin{tabular} {c}
\epsfig{file=scan-rbt-DzKm-comp-DalitzGLWADSRPMHIST.eps,width=0.85\linewidth} \\
\epsfig{file=scan-rbt-DstKm-comp-DalitzGLWADSRPMHIST.eps,width=0.85\linewidth} \\
\epsfig{file=scan-gammat-comp-DalitzGLWADSRPMHIST.eps,width=0.85\linewidth} 
\end{tabular}
\end{center}
\caption{(color online). Comparison of $1-\CL$ as a function of \rb (top), \rbst (middle), and \g (bottom) for all \B decay channels combined with the 
GGSZ method only, the combination with the GLW measurements, and the global combination, 
including statistical and systematic uncertainties.
The horizontal lines represent the one-, two-, three- and four-standard-deviation \CL.
\label{fig:scan-comp-rb+gamma}
}
\end{figure}





\begin{table}[htb]
\caption{\label{tab:polarresults} $68.3\%$ and $95.5\%$ 1-dimensional \CL regions,
equivalent to one- and two-standard-deviation intervals,
for \g, \deltabdeltabst, \deltas, \rbrbst, and \krs,
including all sources of uncertainty, obtained from the combination of GGSZ, GLW, and ADS measurements.
The combined results are compared to those obtained using the GGSZ measurements only, taken from Ref.~\cite{ref:GGSZ2010}.
The results for \g, \deltabdeltabst, and \deltas\ are given modulo 
a $180^\circ$ phase.
}
\begin{center}
\begin{ruledtabular}
\begin{tabular}{lrrrr}
Parameter            & \multicolumn{2}{c}{$68.3\%$ \CL}  & \multicolumn{2}{c}{$95.5\%$ \CL} \\ 
                     & Combination & GGSZ & Combination & GGSZ \\ [0.035in] \hline
 \noalign{\vskip3pt}
\g $(^\circ)$         & $69^{+17}_{-16}$       &  $68^{+15}_{-14}$     & $[41,102]$   & $[39,98]$ \\
\rb $(\%)$           & $9.2 ^{+1.3}_{-1.2}$   &  $9.6 \pm 2.9$      & $[6.0,12.6]$ & $[3.7,15.5]$ \\
\rbst $(\%)$         & $10.6^{+1.9}_{-3.6}$   &  $13.3^{+4.2}_{-3.9}$  & $[3.0,14.7]$ & $[4.9,21.5]$ \\
\krs $(\%)$          & $14.3^{+4.8}_{-4.9}$   &  $14.9^{+6.6}_{-6.2}$  & $[3.3,25.1]$ & $< 28.0$ \\
\deltab   $(^\circ)$  & $105^{+16}_{-17}$      &  $119^{+19}_{-20}$    & $[72,139]$   & $[75,157]$ \\
\deltabst $(^\circ)$  & $-66^{+21}_{-31}$      &  $-82\pm21$        & $[-132,-26]$ & $[-124,-38]$ \\
\deltas   $(^\circ)$  & $101\pm43$          &  $111\pm32$        & $[32,166]$   & $[42,178]$ \\
\end{tabular}
\end{ruledtabular}
\end{center}
\end{table}


The significance of direct \CP violation is obtained by evaluating $1-\CL$ for the most probable \CP conserving 
point, i.e., the set of hadronic parameters \uvec with $\g=0$. Including 
statistical and systematic uncertainties, we obtain $1-\CL=3.4\times 10^{-7},\ 2.5\times 10^{-3}$, and $3.6\times 10^{-2}$,
corresponding to $5.1$, $3.0$, and $2.1$ standard deviations, for
$\Bpm\to\D\Kpm$, $\Bpm\to\Dstar\Kpm$, and $\Bpm\to\D\Kstarpm$ decays, respectively.
For the combination of the three decay modes we obtain $1-\CL=3.1\times 10^{-9}$, corresponding to $5.9$ standard deviations.
For comparison,
the corresponding significances with the GGSZ method alone are
$2.9$, $2.8$, $1.5$, and $4.0$ standard deviations~\cite{ref:CPsignificanceFix},
while with the GGSZ and GLW combination they are
$4.8$, $2.7$, $1.8$, and $5.4$, respectively.

The frequentist procedure used to obtain \g and the hadronic parameters \uvec
is not guaranteed to have perfect coverage, especially 
for low values of \rbrbst, \rs.
This is due to the treatment of nuisance
parameters~\cite{ref:woodroofe}.
Instead of scanning the entire parameter
space defined by \g and \uvec (seven dimensions), we perform one-dimensional scans,
in which, during MC generation, the nuisance parameters are set to their re-optimized
best-fit values at each scan point. 
In order to evaluate the coverage properties of our procedure, we generate 
more than $10^9$ samples 
with true values of $(\g,\uvec)$ set to their
best fit values, $(\g_{\mathrm{best}},\uvec_{\mathrm{best}})$,
as given in Table~\ref{tab:polarresults}. For each generated experiment, we determine
$1-\CL'$ at $\g_0 = \g_{\mathrm{best}}$, as done previously with the actual data sample 
using the Monte Carlo simulation method. 
The statistical coverage $\alpha$, defined as the probability for the true value of \g ($\g_0$) to be inside the given $1-\CL$ interval, 
is evaluated as the fraction of experiments with $1-\CL'$ larger than $1-\CL$. We obtain $\alpha=0.679\pm0.005\ (0.955\pm0.002)$
for the combination, and $\alpha = 0.670\pm0.005\ (0.950\pm0.002)$ for the GGSZ method alone, for $\CL=0.683\ (0.954)$,  respectively.
For comparison purposes, the corresponding values using the Prob method are $\alpha=0.641\pm0.005\ (0.941\pm0.003)$ and $\alpha = 0.609\pm0.005\ (0.920\pm0.003)$.
While the Prob method tends to underestimate the confidence intervals, the Monte Carlo simulation method provides intervals with correct coverage, especially
for the combination where the magnitude ratios between the suppressed and favored decays have more stringent constraints.


